Do Kernel and Neural Embeddings Help in Training and Generalization?

Recent results on optimization and generalization properties of neural networks showed that in a simple two-layer network, the alignment of the labels to the eigenvectors of the corresponding Gram matrix determines the convergence of the optimization during training. Such analyses also provide upper bounds on the generalization error. We experimentally investigate the implications of these results to deeper networks via embeddings. We regard the layers preceding the final hidden layer as producing different representations of the input data which are then fed to the two-layer model. We show that these representations improve both optimization and generalization. In particular, we investigate three kernel representations when fed to the final hidden layer: the Gaussian kernel and its approximation by random Fourier features, kernels designed to imitate representations produced by neural networks and finally an optimal kernel designed to align the data with target labels. The approximated representations induced by these kernels are fed to the neural network and the optimization and generalization properties of the final model are evaluated and compared.

==> comments.tex <==
\section{Answers to the reviewers’ comments}
We would like to thank all the reviewers for their effort in providing comprehensive comments about our work. In what follows we have included detailed answers to all comments.

\subsection{reviewer \#1}
\paragraph{Comment 1.} The authors say:
"Finally we ask the question: What is the optimal representation for optimization and generalization? The work of [1] suggests seeking a representation which makes the label vector align best to the top eigenvectors of the associated Gram matrix."
What I understand from [1] is that alignment with the top eigenvectors only answers the optimization problem not the generalization one.
\paragraph{Answer.} We agree with the reviewer's point about optimization and generalization. Specifically, in \cite{Arora19} there are two main results: i) For a set of labels $\mathbf{y}$, if they align with the top eigenvectors, then gradient descent converges quickly. ii) A complexity measure of data is provided that one can use to predict the test accuracy of the learned neural network. This measure to be computed on the given data, can clearly distinguish between true labels and
random labels. Therefore, in the revised version of the paper we have clarified the reviewer's point in the main text when talking about the alignment. 
\paragraph{Comment 2.} The authors say "What is the optimal representation for optimization and generalization?"
I agree with reviewer 3 that the term optimality should be used with care. [1] only obtained a generalization bound, i.e. an upper bound. Therefore optimizing their criteria does not mean finding the optimal representation. 
\paragraph{Answer.} We agree with reviewer's comment about the term optimality and we have revised the text of the paper accordingly.

\paragraph{Comment 3.}  My comment that alignment with the top eigenvectors is only related to optimization affects also the following sentence:

1) We use the criterion suggested in these papers as a proxy for aligning the label vector to the top eigenvectors and compute the representation so produced. Indeed we observe that this representation provides the best results for training and generalization.

2) [1] show that both training and generalization become better if the label vector y aligns with the eigenvectors corresponding to the top eigenvalues of $H^\infty$.

3) We can therefore improve both training and generalization with kernels since we can get better alignment of the eigenvectors belonging the largest eigenvalues and the target labels.
\paragraph{Answer.} We agree with reviewer's comments on the alignment, and in the revised version of the paper we have changed the text accordingly. 
\paragraph{Comment 4.} In Section 3.1.2 the authors say that "Since for the infinite dimensional case we do not have access to the feature maps, we use K(xi; xj) in the closed form of Gram Matrix and normalization is not done."
However, according to Section 3.1 of [1], normalization is necessary for the results of [1] to hold. In fact, without normalization $x_i^T x_j$ may be greater than one or less than minus one and arccos ($x_i^T x_j$) would not be defined. The authors can simply normalize data in the feature space of a kernel by the following formula.

$\tilde{k}(x,z) = <\phi(x)/\norm{\phi(x)}, \phi(z)/\norm{\phi(z)}> = k(x,z)/ (\sqrt{k(x,x)} \sqrt{k(z,z)})$

which does not require direct access to the feature space. See also exercise 2.18 of the following book:

Schalkopf, Bernhard, Alexander J. Smola, and Francis Bach. Learning with kernels: support vector machines, regularization, optimization, and beyond. MIT press, 2002.
In fact, for Gaussian kernels since $k(x,x) = 1$, the images of input data in the feature space are already normalized. So, the experiment of this section is correct but the writing should be corrected.

\paragraph{Answer.} We appreciate the comment on normalization. In the revised version we have corrected the writing. 
\paragraph{Comment 5.} The authors report $y^T (H^\infty)^{-1} y$ as their measure of generalization. This is not a good choice since it does not show the relation with classification error. As shown in Eq.4 of [1], an upper bound for the generalization error is:
$\sqrt{2y^T (H^\infty)^{-1} y /n}$
where n is the number of samples used in constructing $H^\infty$.
Please always report this upper bound which is very often more than one (but not always).
In addition, please mention the value $n$ clearly in the reports (E.g. Table 2).
From the results reported in Table 2 and my experience with this measure, I guess that the authors should have used 1000 samples for each class (At least for MNIST).
This modification should be applied to Table 3 as well.
\paragraph{Answer.} We agree with the reviewer's comment about the generalization upper bound. In the revised version, we have reported the upper bounds based on the formula mentioned by the reviewer together with values of $n$. 
\paragraph{Comment 6.} The authors say "We observe that for a fairly small number of epochs (up to 5,000) we obtain very sophisticated neural embeddings"
Considering that the optimization is performed by gradient descent (i.e. full batch), 5,000 epochs is an extremely high number.
\paragraph{Answer.} We agree with the reviewer that 5000 is a high number of epochs in our setting. In the revised version, we have removed the corresponding section as suggested in comment 8.
\paragraph{Comment 7.} There are many figures in the paper, making reading the paper tedious. I suggest aggregating related figures in large figures. For example, it is better to combine Figures 6, 7, and 8 in a large figure. This comment applies to all figures and the mentioned one was an example.
\paragraph{Answer.} We thank the reviewer for the suggestion. In the revised version, we have aggregated related figures.
\paragraph{Comment 8.} Considering the high length of the paper and repetitive experiments, I suggest that the Section "3.2.3 Dynamics of neural embeddings" be omitted and it be mentioned at the end of the previous section that similar results would have been obtained if the training process took 5,000 epochs. I leave the decision to the authors.
\paragraph{Answer.} We have removed the mentioned section in the revised version.
\paragraph{Comment 9.} The term "Model-free kernel learning" does not seem true. The authors are using multiple kernel learning, a combination of 7 Gaussian kernels.
\paragraph{Answer.} We agree with the reviewer about the term model-free kernel learning. In the revised version, we use the more appropriate term "multiple kernel learning" as suggested by the reviewer.
\paragraph{Comment 10.}  The authors say "We use 7 Gaussian kernels as the base kernels". Details of these base kernels should be mentioned.
\paragraph{Answer.} Similar to the experiments in \cite{CortesMohri2012}, we use 7 different values for the parameter $\gamma$ in the Gaussian kernel. We have added the details of these values in the revised version. 
\paragraph{Comment 11.} Overall, I find the paper very tedious. All experiments before kernel alignment show that if the parameters of fixed kernels were chosen appropriately, then it would improve both optimization and generalization. I believe that this improvement is a result of choosing appropriate parameters for the kernels. E.g. it is clear that a Gaussian kernel with $\gamma = 1000$ would not generalize. When the paper becomes so boring that the reader have stopped reading it, the more interesting topic of kernel alignment begins. I suggest the authors to consider this comment and make the material of the previous sections more concise.
\paragraph{Answer.} We thank the reviewer for the comment. In the revised version we have removed section 3.2.3 as suggested by the reviewer, and added the point on appropriate kernel parameters. We have also aggregated sections 3.1, 3.1.1 and 3.1.2 to make the previous sections smaller.
\paragraph{Comment 12.} Considering the size of the paper, in the next revision, please provide us with a diff file in which the changes to the current version are shown with red (for removal) and green (for addition) colors so that the reviewers can check the changes without reading the whole paper.
\paragraph{Answer.} We have provided a diff file in our submission to highlight the changes. 















